Measurement of the W boson helicity in top quark decays using 5.4 fb^-1 of ppbar collision data

We present a measurement of the helicity of the W boson produced in top quark decays using ttbar decays in the l+jets and dilepton final states selected from a sample of 5.4 fb^-1 of collisions recorded using the D0 detector at the Fermilab Tevatron ppbar collider. We measure the fractions of longitudinal and right-handed W bosons to be f_0 = 0.669 +- 0.102 [ +- 0.078 (stat.) +- 0.065 (syst.)] and f_+ = 0.023 +- 0.053 [+- 0.041 (stat.) +- 0.034 (syst.)], respectively. This result is consistent at the 98% level with the standard model. A measurement with f_0 fixed to the value from the standard model yields f_+ = 0.010 +- 0.037 [+- 0.022 (stat.) +- 0.030 (syst.) ].

==> acknowledgement_paragraph_r2.tex <==
% acknowledgement_paragraph_r2.tex                          2/4/10
%
We thank the staffs at Fermilab and collaborating institutions, 
and acknowledge support from the 
DOE and NSF (USA);
CEA and CNRS/IN2P3 (France);
FASI, Rosatom and RFBR (Russia);
CNPq, FAPERJ, FAPESP and FUNDUNESP (Brazil);
DAE and DST (India);
Colciencias (Colombia);
CONACyT (Mexico);
KRF and KOSEF (Korea);
CONICET and UBACyT (Argentina);
FOM (The Netherlands);
STFC and the Royal Society (United Kingdom);
MSMT and GACR (Czech Republic);
CRC Program and NSERC (Canada);
BMBF and DFG (Germany);
SFI (Ireland);
The Swedish Research Council (Sweden);
and
CAS and CNSF (China).
%


==> list_of_authors_r2.tex <==
% LIST_OF_AUTHORS_R2.TEX      4 Feb 2010                    
%
% remove these 3 lines before journal submittal.
\centerline{author list dated 4 Feb 2010}
% end removal before journal submittal
%
\author{V.M.~Abazov$^{36}$}
\author{B.~Abbott$^{74}$}
\author{M.~Abolins$^{63}$}
\author{B.S.~Acharya$^{29}$}
\author{M.~Adams$^{49}$}
\author{T.~Adams$^{47}$}
\author{E.~Aguilo$^{6}$}
\author{G.D.~Alexeev$^{36}$}
\author{G.~Alkhazov$^{40}$}
\author{A.~Alton$^{62,a}$}
\author{G.~Alverson$^{61}$}
\author{G.A.~Alves$^{2}$}
\author{L.S.~Ancu$^{35}$}
\author{M.~Aoki$^{48}$}
\author{Y.~Arnoud$^{14}$}
\author{M.~Arov$^{58}$}
\author{A.~Askew$^{47}$}
\author{B.~{\AA}sman$^{41}$}
\author{O.~Atramentov$^{66}$}
\author{C.~Avila$^{8}$}
\author{J.~BackusMayes$^{81}$}
\author{F.~Badaud$^{13}$}
\author{L.~Bagby$^{48}$}
\author{B.~Baldin$^{48}$}
\author{D.V.~Bandurin$^{47}$}
\author{S.~Banerjee$^{29}$}
\author{E.~Barberis$^{61}$}
\author{A.-F.~Barfuss$^{15}$}
\author{P.~Baringer$^{56}$}
\author{J.~Barreto$^{2}$}
\author{J.F.~Bartlett$^{48}$}
\author{U.~Bassler$^{18}$}
\author{S.~Beale$^{6}$}
\author{A.~Bean$^{56}$}
\author{M.~Begalli$^{3}$}
\author{M.~Begel$^{72}$}
\author{C.~Belanger-Champagne$^{41}$}
\author{L.~Bellantoni$^{48}$}
\author{J.A.~Benitez$^{63}$}
\author{S.B.~Beri$^{27}$}
\author{G.~Bernardi$^{17}$}
\author{R.~Bernhard$^{22}$}
\author{I.~Bertram$^{42}$}
\author{M.~Besan\c{c}on$^{18}$}
\author{R.~Beuselinck$^{43}$}
\author{V.A.~Bezzubov$^{39}$}
\author{P.C.~Bhat$^{48}$}
\author{V.~Bhatnagar$^{27}$}
\author{G.~Blazey$^{50}$}
\author{S.~Blessing$^{47}$}
\author{K.~Bloom$^{65}$}
\author{A.~Boehnlein$^{48}$}
\author{D.~Boline$^{60}$}
\author{T.A.~Bolton$^{57}$}
\author{E.E.~Boos$^{38}$}
\author{G.~Borissov$^{42}$}
\author{T.~Bose$^{60}$}
\author{A.~Brandt$^{77}$}
\author{R.~Brock$^{63}$}
\author{G.~Brooijmans$^{69}$}
\author{A.~Bross$^{48}$}
\author{D.~Brown$^{19}$}
\author{X.B.~Bu$^{7}$}
\author{D.~Buchholz$^{51}$}
\author{M.~Buehler$^{80}$}
\author{V.~Buescher$^{24}$}
\author{V.~Bunichev$^{38}$}
\author{S.~Burdin$^{42,b}$}
\author{T.H.~Burnett$^{81}$}
\author{C.P.~Buszello$^{43}$}
\author{P.~Calfayan$^{25}$}
\author{B.~Calpas$^{15}$}
\author{S.~Calvet$^{16}$}
\author{E.~Camacho-P\'erez$^{33}$}
\author{J.~Cammin$^{70}$}
\author{M.A.~Carrasco-Lizarraga$^{33}$}
\author{E.~Carrera$^{47}$}
\author{B.C.K.~Casey$^{48}$}
\author{H.~Castilla-Valdez$^{33}$}
\author{S.~Chakrabarti$^{71}$}
\author{D.~Chakraborty$^{50}$}
\author{K.M.~Chan$^{54}$}
\author{A.~Chandra$^{79}$}
\author{G.~Chen$^{56}$}
\author{S.~Chevalier-Th\'ery$^{18}$}
\author{D.K.~Cho$^{76}$}
\author{S.W.~Cho$^{31}$}
\author{S.~Choi$^{32}$}
\author{B.~Choudhary$^{28}$}
\author{T.~Christoudias$^{43}$}
\author{S.~Cihangir$^{48}$}
\author{D.~Claes$^{65}$}
\author{J.~Clutter$^{56}$}
\author{M.~Cooke$^{48}$}
\author{W.E.~Cooper$^{48}$}
\author{M.~Corcoran$^{79}$}
\author{F.~Couderc$^{18}$}
\author{M.-C.~Cousinou$^{15}$}
\author{D.~Cutts$^{76}$}
\author{M.~{\'C}wiok$^{30}$}
\author{A.~Das$^{45}$}
\author{G.~Davies$^{43}$}
\author{K.~De$^{77}$}
\author{S.J.~de~Jong$^{35}$}
\author{E.~De~La~Cruz-Burelo$^{33}$}
\author{K.~DeVaughan$^{65}$}
\author{F.~D\'eliot$^{18}$}
\author{M.~Demarteau$^{48}$}
\author{R.~Demina$^{70}$}
\author{D.~Denisov$^{48}$}
\author{S.P.~Denisov$^{39}$}
\author{S.~Desai$^{48}$}
\author{H.T.~Diehl$^{48}$}
\author{M.~Diesburg$^{48}$}
\author{A.~Dominguez$^{65}$}
\author{T.~Dorland$^{81}$}
\author{A.~Dubey$^{28}$}
\author{L.V.~Dudko$^{38}$}
\author{L.~Duflot$^{16}$}
\author{D.~Duggan$^{66}$}
\author{A.~Duperrin$^{15}$}
\author{S.~Dutt$^{27}$}
\author{A.~Dyshkant$^{50}$}
\author{M.~Eads$^{65}$}
\author{D.~Edmunds$^{63}$}
\author{J.~Ellison$^{46}$}
\author{V.D.~Elvira$^{48}$}
\author{Y.~Enari$^{17}$}
\author{S.~Eno$^{59}$}
\author{H.~Evans$^{52}$}
\author{A.~Evdokimov$^{72}$}
\author{V.N.~Evdokimov$^{39}$}
\author{G.~Facini$^{61}$}
\author{A.V.~Ferapontov$^{76}$}
\author{T.~Ferbel$^{59,70}$}
\author{F.~Fiedler$^{24}$}
\author{F.~Filthaut$^{35}$}
\author{W.~Fisher$^{63}$}
\author{H.E.~Fisk$^{48}$}
\author{M.~Fortner$^{50}$}
\author{H.~Fox$^{42}$}
\author{S.~Fuess$^{48}$}
\author{T.~Gadfort$^{72}$}
\author{A.~Garcia-Bellido$^{70}$}
\author{V.~Gavrilov$^{37}$}
\author{P.~Gay$^{13}$}
\author{W.~Geist$^{19}$}
\author{W.~Geng$^{15,63}$}
\author{D.~Gerbaudo$^{67}$}
\author{C.E.~Gerber$^{49}$}
\author{Y.~Gershtein$^{66}$}
\author{D.~Gillberg$^{6}$}
\author{G.~Ginther$^{48,70}$}
\author{G.~Golovanov$^{36}$}
\author{B.~G\'{o}mez$^{8}$}
\author{A.~Goussiou$^{81}$}
\author{P.D.~Grannis$^{71}$}
\author{S.~Greder$^{19}$}
\author{H.~Greenlee$^{48}$}
\author{Z.D.~Greenwood$^{58}$}
\author{E.M.~Gregores$^{4}$}
\author{G.~Grenier$^{20}$}
\author{Ph.~Gris$^{13}$}
\author{J.-F.~Grivaz$^{16}$}
\author{A.~Grohsjean$^{18}$}
\author{S.~Gr\"unendahl$^{48}$}
\author{M.W.~Gr{\"u}newald$^{30}$}
\author{F.~Guo$^{71}$}
\author{J.~Guo$^{71}$}
\author{G.~Gutierrez$^{48}$}
\author{P.~Gutierrez$^{74}$}
\author{A.~Haas$^{69,c}$}
\author{P.~Haefner$^{25}$}
\author{S.~Hagopian$^{47}$}
\author{J.~Haley$^{61}$}
\author{I.~Hall$^{63}$}
\author{L.~Han$^{7}$}
\author{K.~Harder$^{44}$}
\author{A.~Harel$^{70}$}
\author{J.M.~Hauptman$^{55}$}
\author{J.~Hays$^{43}$}
\author{T.~Hebbeker$^{21}$}
\author{D.~Hedin$^{50}$}
\author{A.P.~Heinson$^{46}$}
\author{U.~Heintz$^{76}$}
\author{C.~Hensel$^{23}$}
\author{I.~Heredia-De~La~Cruz$^{33}$}
\author{K.~Herner$^{62}$}
\author{G.~Hesketh$^{61}$}
\author{M.D.~Hildreth$^{54}$}
\author{R.~Hirosky$^{80}$}
\author{T.~Hoang$^{47}$}
\author{J.D.~Hobbs$^{71}$}
\author{B.~Hoeneisen$^{12}$}
\author{M.~Hohlfeld$^{24}$}
\author{S.~Hossain$^{74}$}
\author{P.~Houben$^{34}$}
\author{Y.~Hu$^{71}$}
\author{Z.~Hubacek$^{10}$}
\author{N.~Huske$^{17}$}
\author{V.~Hynek$^{10}$}
\author{I.~Iashvili$^{68}$}
\author{R.~Illingworth$^{48}$}
\author{A.S.~Ito$^{48}$}
\author{S.~Jabeen$^{76}$}
\author{M.~Jaffr\'e$^{16}$}
\author{S.~Jain$^{68}$}
\author{D.~Jamin$^{15}$}
\author{R.~Jesik$^{43}$}
\author{K.~Johns$^{45}$}
\author{C.~Johnson$^{69}$}
\author{M.~Johnson$^{48}$}
\author{D.~Johnston$^{65}$}
\author{A.~Jonckheere$^{48}$}
\author{P.~Jonsson$^{43}$}
\author{A.~Juste$^{48,d}$}
\author{E.~Kajfasz$^{15}$}
\author{D.~Karmanov$^{38}$}
\author{P.A.~Kasper$^{48}$}
\author{I.~Katsanos$^{65}$}
\author{R.~Kehoe$^{78}$}
\author{S.~Kermiche$^{15}$}
\author{N.~Khalatyan$^{48}$}
\author{A.~Khanov$^{75}$}
\author{A.~Kharchilava$^{68}$}
\author{Y.N.~Kharzheev$^{36}$}
\author{D.~Khatidze$^{76}$}
\author{M.H.~Kirby$^{51}$}
\author{M.~Kirsch$^{21}$}
\author{J.M.~Kohli$^{27}$}
\author{A.V.~Kozelov$^{39}$}
\author{J.~Kraus$^{63}$}
\author{A.~Kumar$^{68}$}
\author{A.~Kupco$^{11}$}
\author{T.~Kur\v{c}a$^{20}$}
\author{V.A.~Kuzmin$^{38}$}
\author{J.~Kvita$^{9}$}
\author{S.~Lammers$^{52}$}
\author{G.~Landsberg$^{76}$}
\author{P.~Lebrun$^{20}$}
\author{H.S.~Lee$^{31}$}
\author{W.M.~Lee$^{48}$}
\author{J.~Lellouch$^{17}$}
\author{L.~Li$^{46}$}
\author{Q.Z.~Li$^{48}$}
\author{S.M.~Lietti$^{5}$}
\author{J.K.~Lim$^{31}$}
\author{D.~Lincoln$^{48}$}
\author{J.~Linnemann$^{63}$}
\author{V.V.~Lipaev$^{39}$}
\author{R.~Lipton$^{48}$}
\author{Y.~Liu$^{7}$}
\author{Z.~Liu$^{6}$}
\author{A.~Lobodenko$^{40}$}
\author{M.~Lokajicek$^{11}$}
\author{P.~Love$^{42}$}
\author{H.J.~Lubatti$^{81}$}
\author{R.~Luna-Garcia$^{33,e}$}
\author{A.L.~Lyon$^{48}$}
\author{A.K.A.~Maciel$^{2}$}
\author{D.~Mackin$^{79}$}
\author{R.~Maga\~na-Villalba$^{33}$}
\author{P.K.~Mal$^{45}$}
\author{S.~Malik$^{65}$}
\author{V.L.~Malyshev$^{36}$}
\author{Y.~Maravin$^{57}$}
\author{J.~Mart\'{\i}nez-Ortega$^{33}$}
\author{R.~McCarthy$^{71}$}
\author{C.L.~McGivern$^{56}$}
\author{M.M.~Meijer$^{35}$}
\author{A.~Melnitchouk$^{64}$}
\author{L.~Mendoza$^{8}$}
\author{D.~Menezes$^{50}$}
\author{P.G.~Mercadante$^{4}$}
\author{M.~Merkin$^{38}$}
\author{A.~Meyer$^{21}$}
\author{J.~Meyer$^{23}$}
\author{N.K.~Mondal$^{29}$}
\author{T.~Moulik$^{56}$}
\author{G.S.~Muanza$^{15}$}
\author{M.~Mulhearn$^{80}$}
\author{E.~Nagy$^{15}$}
\author{M.~Naimuddin$^{28}$}
\author{M.~Narain$^{76}$}
\author{R.~Nayyar$^{28}$}
\author{H.A.~Neal$^{62}$}
\author{J.P.~Negret$^{8}$}
\author{P.~Neustroev$^{40}$}
\author{H.~Nilsen$^{22}$}
\author{S.F.~Novaes$^{5}$}
\author{T.~Nunnemann$^{25}$}
\author{G.~Obrant$^{40}$}
\author{D.~Onoprienko$^{57}$}
\author{J.~Orduna$^{33}$}
\author{N.~Osman$^{43}$}
\author{J.~Osta$^{54}$}
\author{G.J.~Otero~y~Garz{\'o}n$^{1}$}
\author{M.~Owen$^{44}$}
\author{M.~Padilla$^{46}$}
\author{M.~Pangilinan$^{76}$}
\author{N.~Parashar$^{53}$}
\author{V.~Parihar$^{76}$}
\author{S.-J.~Park$^{23}$}
\author{S.K.~Park$^{31}$}
\author{J.~Parsons$^{69}$}
\author{R.~Partridge$^{76}$}
\author{N.~Parua$^{52}$}
\author{A.~Patwa$^{72}$}
\author{B.~Penning$^{48}$}
\author{M.~Perfilov$^{38}$}
\author{K.~Peters$^{44}$}
\author{Y.~Peters$^{44}$}
\author{P.~P\'etroff$^{16}$}
\author{R.~Piegaia$^{1}$}
\author{J.~Piper$^{63}$}
\author{M.-A.~Pleier$^{72}$}
\author{P.L.M.~Podesta-Lerma$^{33,f}$}
\author{V.M.~Podstavkov$^{48}$}
\author{M.-E.~Pol$^{2}$}
\author{P.~Polozov$^{37}$}
\author{A.V.~Popov$^{39}$}
\author{M.~Prewitt$^{79}$}
\author{D.~Price$^{52}$}
\author{S.~Protopopescu$^{72}$}
\author{J.~Qian$^{62}$}
\author{A.~Quadt$^{23}$}
\author{B.~Quinn$^{64}$}
\author{M.S.~Rangel$^{16}$}
\author{K.~Ranjan$^{28}$}
\author{P.N.~Ratoff$^{42}$}
\author{I.~Razumov$^{39}$}
\author{P.~Renkel$^{78}$}
\author{P.~Rich$^{44}$}
\author{M.~Rijssenbeek$^{71}$}
\author{I.~Ripp-Baudot$^{19}$}
\author{F.~Rizatdinova$^{75}$}
\author{M.~Rominsky$^{48}$}
\author{C.~Royon$^{18}$}
\author{P.~Rubinov$^{48}$}
\author{R.~Ruchti$^{54}$}
\author{G.~Safronov$^{37}$}
\author{G.~Sajot$^{14}$}
\author{A.~S\'anchez-Hern\'andez$^{33}$}
\author{M.P.~Sanders$^{25}$}
\author{B.~Sanghi$^{48}$}
\author{G.~Savage$^{48}$}
\author{L.~Sawyer$^{58}$}
\author{T.~Scanlon$^{43}$}
\author{D.~Schaile$^{25}$}
\author{R.D.~Schamberger$^{71}$}
\author{Y.~Scheglov$^{40}$}
\author{H.~Schellman$^{51}$}
\author{T.~Schliephake$^{26}$}
\author{S.~Schlobohm$^{81}$}
\author{C.~Schwanenberger$^{44}$}
\author{R.~Schwienhorst$^{63}$}
\author{J.~Sekaric$^{56}$}
\author{H.~Severini$^{74}$}
\author{E.~Shabalina$^{23}$}
\author{V.~Shary$^{18}$}
\author{A.A.~Shchukin$^{39}$}
\author{R.K.~Shivpuri$^{28}$}
\author{V.~Simak$^{10}$}
\author{V.~Sirotenko$^{48}$}
\author{P.~Skubic$^{74}$}
\author{P.~Slattery$^{70}$}
\author{D.~Smirnov$^{54}$}
\author{G.R.~Snow$^{65}$}
\author{J.~Snow$^{73}$}
\author{S.~Snyder$^{72}$}
\author{S.~S{\"o}ldner-Rembold$^{44}$}
\author{L.~Sonnenschein$^{21}$}
\author{A.~Sopczak$^{42}$}
\author{M.~Sosebee$^{77}$}
\author{K.~Soustruznik$^{9}$}
\author{B.~Spurlock$^{77}$}
\author{J.~Stark$^{14}$}
\author{V.~Stolin$^{37}$}
\author{D.A.~Stoyanova$^{39}$}
\author{M.A.~Strang$^{68}$}
\author{E.~Strauss$^{71}$}
\author{M.~Strauss$^{74}$}
\author{R.~Str{\"o}hmer$^{25}$}
\author{D.~Strom$^{49}$}
\author{L.~Stutte$^{48}$}
\author{P.~Svoisky$^{35}$}
\author{M.~Takahashi$^{44}$}
\author{A.~Tanasijczuk$^{1}$}
\author{W.~Taylor$^{6}$}
\author{B.~Tiller$^{25}$}
\author{M.~Titov$^{18}$}
\author{V.V.~Tokmenin$^{36}$}
\author{D.~Tsybychev$^{71}$}
\author{B.~Tuchming$^{18}$}
\author{C.~Tully$^{67}$}
\author{P.M.~Tuts$^{69}$}
\author{R.~Unalan$^{63}$}
\author{L.~Uvarov$^{40}$}
\author{S.~Uvarov$^{40}$}
\author{S.~Uzunyan$^{50}$}
\author{R.~Van~Kooten$^{52}$}
\author{W.M.~van~Leeuwen$^{34}$}
\author{N.~Varelas$^{49}$}
\author{E.W.~Varnes$^{45}$}
\author{I.A.~Vasilyev$^{39}$}
\author{P.~Verdier$^{20}$}
\author{L.S.~Vertogradov$^{36}$}
\author{M.~Verzocchi$^{48}$}
\author{M.~Vesterinen$^{44}$}
\author{D.~Vilanova$^{18}$}
\author{P.~Vint$^{43}$}
\author{P.~Vokac$^{10}$}
\author{H.D.~Wahl$^{47}$}
\author{M.H.L.S.~Wang$^{70}$}
\author{J.~Warchol$^{54}$}
\author{G.~Watts$^{81}$}
\author{M.~Wayne$^{54}$}
\author{G.~Weber$^{24}$}
\author{M.~Weber$^{48,g}$}
\author{M.~Wetstein$^{59}$}
\author{A.~White$^{77}$}
\author{D.~Wicke$^{24}$}
\author{M.R.J.~Williams$^{42}$}
\author{G.W.~Wilson$^{56}$}
\author{S.J.~Wimpenny$^{46}$}
\author{M.~Wobisch$^{58}$}
\author{D.R.~Wood$^{61}$}
\author{T.R.~Wyatt$^{44}$}
\author{Y.~Xie$^{48}$}
\author{C.~Xu$^{62}$}
\author{S.~Yacoob$^{51}$}
\author{R.~Yamada$^{48}$}
\author{W.-C.~Yang$^{44}$}
\author{T.~Yasuda$^{48}$}
\author{Y.A.~Yatsunenko$^{36}$}
\author{Z.~Ye$^{48}$}
\author{H.~Yin$^{7}$}
\author{K.~Yip$^{72}$}
\author{H.D.~Yoo$^{76}$}
\author{S.W.~Youn$^{48}$}
\author{J.~Yu$^{77}$}
\author{S.~Zelitch$^{80}$}
\author{T.~Zhao$^{81}$}
\author{B.~Zhou$^{62}$}
\author{J.~Zhu$^{71}$}
\author{M.~Zielinski$^{70}$}
\author{D.~Zieminska$^{52}$}
\author{L.~Zivkovic$^{69}$}

\affiliation{\vspace{0.1 in}(The D\O\ Collaboration)\vspace{0.1 in}}
\affiliation{$^{1}$Universidad de Buenos Aires, Buenos Aires, Argentina}
\affiliation{$^{2}$LAFEX, Centro Brasileiro de Pesquisas F{\'\i}sicas,
                Rio de Janeiro, Brazil}
\affiliation{$^{3}$Universidade do Estado do Rio de Janeiro,
                Rio de Janeiro, Brazil}
\affiliation{$^{4}$Universidade Federal do ABC,
                Santo Andr\'e, Brazil}
\affiliation{$^{5}$Instituto de F\'{\i}sica Te\'orica, Universidade Estadual
                Paulista, S\~ao Paulo, Brazil}
\affiliation{$^{6}$Simon Fraser University, Burnaby, British Columbia, Canada;
                and York University, Toronto, Ontario, Canada}
\affiliation{$^{7}$University of Science and Technology of China,
                Hefei, People's Republic of China}
\affiliation{$^{8}$Universidad de los Andes, Bogot\'{a}, Colombia}
\affiliation{$^{9}$Center for Particle Physics, Charles University,
                Faculty of Mathematics and Physics, Prague, Czech Republic}
\affiliation{$^{10}$Czech Technical University in Prague,
                Prague, Czech Republic}
\affiliation{$^{11}$Center for Particle Physics, Institute of Physics,
                Academy of Sciences of the Czech Republic,
                Prague, Czech Republic}
\affiliation{$^{12}$Universidad San Francisco de Quito, Quito, Ecuador}
\affiliation{$^{13}$LPC, Universit\'e Blaise Pascal, CNRS/IN2P3,
                Clermont, France}
\affiliation{$^{14}$LPSC, Universit\'e Joseph Fourier Grenoble 1,
                CNRS/IN2P3, Institut National Polytechnique de Grenoble,
                Grenoble, France}
\affiliation{$^{15}$CPPM, Aix-Marseille Universit\'e, CNRS/IN2P3,
                Marseille, France}
\affiliation{$^{16}$LAL, Universit\'e Paris-Sud, IN2P3/CNRS, Orsay, France}
\affiliation{$^{17}$LPNHE, Universit\'es Paris VI and VII, CNRS/IN2P3,
                Paris, France}
\affiliation{$^{18}$CEA, Irfu, SPP, Saclay, France}
\affiliation{$^{19}$IPHC, Universit\'e de Strasbourg, CNRS/IN2P3,
                Strasbourg, France}
\affiliation{$^{20}$IPNL, Universit\'e Lyon 1, CNRS/IN2P3,
                Villeurbanne, France and Universit\'e de Lyon, Lyon, France}
\affiliation{$^{21}$III. Physikalisches Institut A, RWTH Aachen University,
                Aachen, Germany}
\affiliation{$^{22}$Physikalisches Institut, Universit{\"a}t Freiburg,
                Freiburg, Germany}
\affiliation{$^{23}$II. Physikalisches Institut, Georg-August-Universit{\"a}t
                G\"ottingen, G\"ottingen, Germany}
\affiliation{$^{24}$Institut f{\"u}r Physik, Universit{\"a}t Mainz,
                Mainz, Germany}
\affiliation{$^{25}$Ludwig-Maximilians-Universit{\"a}t M{\"u}nchen,
                M{\"u}nchen, Germany}
\affiliation{$^{26}$Fachbereich Physik, University of Wuppertal,
                Wuppertal, Germany}
\affiliation{$^{27}$Panjab University, Chandigarh, India}
\affiliation{$^{28}$Delhi University, Delhi, India}
\affiliation{$^{29}$Tata Institute of Fundamental Research, Mumbai, India}
\affiliation{$^{30}$University College Dublin, Dublin, Ireland}
\affiliation{$^{31}$Korea Detector Laboratory, Korea University, Seoul, Korea}
\affiliation{$^{32}$SungKyunKwan University, Suwon, Korea}
\affiliation{$^{33}$CINVESTAV, Mexico City, Mexico}
\affiliation{$^{34}$FOM-Institute NIKHEF and University of Amsterdam/NIKHEF,
                Amsterdam, The Netherlands}
\affiliation{$^{35}$Radboud University Nijmegen/NIKHEF,
                Nijmegen, The Netherlands}
\affiliation{$^{36}$Joint Institute for Nuclear Research, Dubna, Russia}
\affiliation{$^{37}$Institute for Theoretical and Experimental Physics,
                Moscow, Russia}
\affiliation{$^{38}$Moscow State University, Moscow, Russia}
\affiliation{$^{39}$Institute for High Energy Physics, Protvino, Russia}
\affiliation{$^{40}$Petersburg Nuclear Physics Institute,
                St. Petersburg, Russia}
\affiliation{$^{41}$Stockholm University, Stockholm, Sweden, and
                Uppsala University, Uppsala, Sweden}
\affiliation{$^{42}$Lancaster University, Lancaster LA1 4YB, United Kingdom}
\affiliation{$^{43}$Imperial College London, London SW7 2AZ, United Kingdom}
\affiliation{$^{44}$The University of Manchester, Manchester M13 9PL,
                 United Kingdom}
\affiliation{$^{45}$University of Arizona, Tucson, Arizona 85721, USA}
\affiliation{$^{46}$University of California Riverside, Riverside,
                     California 92521, USA}
\affiliation{$^{47}$Florida State University, Tallahassee, Florida 32306, USA}
\affiliation{$^{48}$Fermi National Accelerator Laboratory,
                Batavia, Illinois 60510, USA}
\affiliation{$^{49}$University of Illinois at Chicago,
                Chicago, Illinois 60607, USA}
\affiliation{$^{50}$Northern Illinois University, DeKalb, Illinois 60115, USA}
\affiliation{$^{51}$Northwestern University, Evanston, Illinois 60208, USA}
\affiliation{$^{52}$Indiana University, Bloomington, Indiana 47405, USA}
\affiliation{$^{53}$Purdue University Calumet, Hammond, Indiana 46323, USA}
\affiliation{$^{54}$University of Notre Dame, Notre Dame, Indiana 46556, USA}
\affiliation{$^{55}$Iowa State University, Ames, Iowa 50011, USA}
\affiliation{$^{56}$University of Kansas, Lawrence, Kansas 66045, USA}
\affiliation{$^{57}$Kansas State University, Manhattan, Kansas 66506, USA}
\affiliation{$^{58}$Louisiana Tech University, Ruston, Louisiana 71272, USA}
\affiliation{$^{59}$University of Maryland, College Park, Maryland 20742, USA}
\affiliation{$^{60}$Boston University, Boston, Massachusetts 02215, USA}
\affiliation{$^{61}$Northeastern University, Boston, Massachusetts 02115, USA}
\affiliation{$^{62}$University of Michigan, Ann Arbor, Michigan 48109, USA}
\affiliation{$^{63}$Michigan State University,
                East Lansing, Michigan 48824, USA}
\affiliation{$^{64}$University of Mississippi,
                University, Mississippi 38677, USA}
\affiliation{$^{65}$University of Nebraska, Lincoln, Nebraska 68588, USA}
\affiliation{$^{66}$Rutgers University, Piscataway, New Jersey 08855, USA}
\affiliation{$^{67}$Princeton University, Princeton, New Jersey 08544, USA}
\affiliation{$^{68}$State University of New York, Buffalo, New York 14260, USA}
\affiliation{$^{69}$Columbia University, New York, New York 10027, USA}
\affiliation{$^{70}$University of Rochester, Rochester, New York 14627, USA}
\affiliation{$^{71}$State University of New York,
                Stony Brook, New York 11794, USA}
\affiliation{$^{72}$Brookhaven National Laboratory, Upton, New York 11973, USA}
\affiliation{$^{73}$Langston University, Langston, Oklahoma 73050, USA}
\affiliation{$^{74}$University of Oklahoma, Norman, Oklahoma 73019, USA}
\affiliation{$^{75}$Oklahoma State University, Stillwater, Oklahoma 74078, USA}
\affiliation{$^{76}$Brown University, Providence, Rhode Island 02912, USA}
\affiliation{$^{77}$University of Texas, Arlington, Texas 76019, USA}
\affiliation{$^{78}$Southern Methodist University, Dallas, Texas 75275, USA}
\affiliation{$^{79}$Rice University, Houston, Texas 77005, USA}
\affiliation{$^{80}$University of Virginia,
                Charlottesville, Virginia 22901, USA}
\affiliation{$^{81}$University of Washington, Seattle, Washington 98195, USA}


==> list_of_visitor_addresses_r2.tex <==
% list_of_visitor_addresses_r2.tex                          2/4/10
%  available symbols are:
%  $\ast, \dag, \ddag, \S, \P, $\|$, $\ast\ast$, \dag\dag, \ddag\ddag ,\#
%
\bibitem[a]{alton}
Visitor from Augustana College, Sioux Falls, SD, USA.
\bibitem[b]{burdin}
Visitor from The University of Liverpool, Liverpool, UK.
\bibitem[c]{haas}
Visitor from SLAC, Menlo Park, CA, USA.
\bibitem[d]{juste}
Visitor from ICREA/IFAE, Barcelona, Spain.
\bibitem[e]{luna-garcia}
Visitor from Centro de Investigacion en Computacion - IPN,
  Mexico City, Mexico.
\bibitem[f]{podesta-lerma}
Visitor from ECFM, Universidad Autonoma de Sinaloa, Culiac\'an, Mexico.
\bibitem[g]{weber}
Visitor from Universit{\"a}t Bern, Bern, Switzerland.
%\bibitem[?]{hooper}
%Visitor from Bradley University, Peoria, IL, USA.
%\bibitem[?]{kozminski}
%Visitor from Lewis University, Romeoville, IL, USA.
%\bibitem[\ddag]{deceased}
%Deceased.

%
\vskip 0.25cm

